Simple parallel and distributed algorithms for spectral graph sparsification

We describe a simple algorithm for spectral graph sparsification, based on iterative computations of weighted spanners and uniform sampling. Leveraging the algorithms of Baswana and Sen for computing spanners, we obtain the first distributed spectral sparsification algorithm. We also obtain a parallel algorithm with improved work and time guarantees. Combining this algorithm with the parallel framework of Peng and Spielman for solving symmetric diagonally dominant linear systems, we get a parallel solver which is much closer to being practical and significantly more efficient in terms of the total work.

==> result.tex <==




\section{The result}


\subsection{The algorithm}



\begin{theorem}
Let $\tilde{G} = \textsc{CombinatorialSparsify}(G)$. Then
$\tilde{G}$
%is a union of $O(\log n)$ trees
has $O(n\log n)$ edges and satisfies $$ \frac{1}{4s_n}  G \preceq \tilde{G} \preceq G,$$ where $s_n$ is defined in Lemma \ref{th:offtreesparsify}.
\end{theorem}
\begin{proof}
The algorithm is recursive. We will number the top level with $i=0$. At every level $0\leq i\leq d$ we can define in the obvious way the graphs $G_i = T_i+H_i$ and $\tilde{G_i},\tilde{H_i}$. Note that the graph $\tilde{H_i}$ results from applying \textsc{SparsifyOffTree} to $H_i$ and $\tilde{G_i}$ from applying \textsc{CombinatorialSparsify} to $G_i$. By construction, we have

\begin{equation} \label{eq:recursivedef}
G_{i+1} =  \tilde{H}_{i} ~~ \textnormal{and}~~ \tilde{G_i} = T_i + (1+1/(16\log n))^{-1} \tilde{G}_{i+1} .
\end{equation}

The depth of the recursion is $d=O(\log n)$ because for every $i$ the number of off-tree edges is reduced by a constant fraction in $i+1$. By a simple bottom-up induction, it follows that $\hat{G}$ has $O(n\log n)$ edges, because it is a sum of a graph with $O(n\log n)$ edges (at the bottom of the recursion) and $O(\log n)$ trees, one per each level.

Using the same induction we show that $\tilde{G}_i \preceq G_i$. For the base of the induction $(j=0)$, it is clear that $\hat{G}_d=G_d\preceq {G}_d $. Now note that since $G_{i+1} = \tilde{H_i}$, the inductive hypothesis gives
$$
\textsc{CombinatorialSparsify}(\tilde{H_i}) \preceq \tilde{H_i}.
$$
and so
$$
\tilde{G_i} \preceq T_i+ (1+1/(16 \log n))^{-1}\tilde{H_i} \preceq T_i + H_i = G_i,
$$
where the second inequality comes from Lemma \ref{th:Hdomination}.


We now focus on the claim that $(1/4s_n) G \preceq \tilde{G}$. Notice that because the depth of recursion $d$ is at most $2\log n$, it is enough to prove that
that $$\left(\frac{1-2/(16\log n)}{1+1/(16\log n)}\right)^{d-i}(1/2s_n) G_{i} \preceq \tilde{G}_{i}.$$
 We will use again bottom-up induction. The base of the induction $(i=d)$ is obvious. Let $x$ be an arbitrary vector. We consider two cases for $x$, based on whether $s_n x^T T_i x  \geq  x^T H_i x$ or not. For the first case, we have
\begin{eqnarray*}
 s_n x^T T_i x  \geq  x^T H_i x  & \Rightarrow &  x^T T_i x \geq (1/2s_n) x^T G_i x \\ & \Rightarrow &  x^T \tilde{G_i} x\geq (1/s_n) x^T G_i x.
\end{eqnarray*}
For the second case, we have
\begin{eqnarray*}
 s_n x^T T_i x \leq  x^T H_i x & \Rightarrow & x^T \tilde{H_i} x\geq (1-2/(16\log n)) x^T {H_i} x  \qquad \textnormal{(by Lemma \ref{th:Htight})} \\
& \Rightarrow & x^T G_{i+1} x \geq (1-2/(16\log n)) x^T H_i x
\qquad \textnormal{(by Eq. \ref{eq:recursivedef}a)} \\
& \Rightarrow & x^T \tilde{G}_{i+1} x \geq \frac{(1-2/(16\log n))^{d-i}}{(1+1/(16\log n))^{d-i-1}}  (1/2s_n) x^T H_i x ~~\textnormal{(by I.H.)}  \\
& \Rightarrow &  x^T \tilde{G}_{i} x \geq \left(\frac{1-2/(16\log n)}{1+1/(16\log n)} \right)^{d-i} (1/2s_n) x^T G_i x.
\end{eqnarray*}
where to get the last line we first multiplied by $(1+1/(16\log n))^{-1}$ and then added $x^T T_{j} x$ on both sides, and finally used equality \ref{eq:recursivedef}.

Combining the two cases proves the claim.
\end{proof}



\begin{comment}
\begin{algo}[h]
\qquad

\textsc{CombinatorialSparsify}
\vspace{0.05cm}

\underline{Input:} Graph $G$

\underline{Output:} Graph $\tilde{G}$
\vspace{0.2cm}

\begin{algorithmic}[1]
\STATE{$\tilde{G}=0$}
\STATE{$i=1; G_i = G$}
\WHILE{$G_i$ has more than $n\log n$ edges}
\STATE{Decompose $G_i$ as $G_i=T_i+H_i$}
\STATE{$\tilde{G} = \tilde{G}i+T_i$}
\STATE{Let $\tilde{H_i}= \textsc{SparsifyOffTree}(H_i)$}
\STATE{$G_{i+1} = (1+1/(16 \log n))^{-1}\tilde{H_i}$}
\ENDWHILE
\STATE{ $\tilde{G} = \tilde{G} + G_i$ \qquad (* The last sparse $G_i$ is just added to $\tilde{G}$ *)}
\end{algorithmic}
%\caption{Sampling}\label{fig:sample}
\end{algo}
\end{comment}

\subsection{Black-box LSST}

Suppose $A$ is a graph with $O(n \log n)$ edges and $B$ is any graph that has the same cuts with $A$.
Let $R_T$ be an R-tree of an MST of $A$. Then
$$
    stretch(A, R_T) = O(n\log^2 n).
$$

Consider an edge $e$ of $A$. There is a unique path of length $O(\log n)$ in $R_T$
that joins the two endpoints of $e=(s,t)$.
The lightest edge in $p_e$ has weight at least $w_e$. Suppose this is not true
and $e'$ is such an edge. Because $s$ and $t$ disconnect if $e'$ is removed in $R_T$,
it follows that $w_e'$ is on the path between $s$ and $t$ in $T$. This is a
contradiction to MST property. Hence
$$
     stretch(e, R_T) = w_e \sum_{e' in p_e} (1/w_e') \leq \log n .
$$
If $e$ is in $T$ it gets routed through smaller edges, so it works too.

Now let $B$ any such graph. Let $e$ an edge in $B$.
$$
     stretch(e, R_T) = w_e \sum_{e' in p_e} R_T
$$
So
$$
     stretch(B, R_T) = \sum_{e\in B} stretch(e,R_T) = \sum_{e' \in R_T} \sum_{e \in B, crossing} {w_e (1/{w_e}')}
$$
which is independent from $B$ because what is crossing is the same. By using the upper bound derived by $A$ we're done.



\subsection{A trace inequality}

\begin{comment}
\begin{lemma}
 Let $A,B$ be positive vectors. For all positive vectors $C<B$, we have
 $$
     \sum_i \frac{2A_i}{B_i} \leq \max \left(\sum_i  \frac{A_i}{C_i}, \sum_i \frac{A_i}{B_i-C_i}\right)
 $$
\end{lemma}
\begin{proof}
  Let $X$ be the vector with $X_i = \frac{A_i}{C_i}$ and $Y$ be the vector with
  $Y_i = \frac{A_i}{B_i-C_i}$. For a vector $X$ we let $X^{\sqrt{}}$ denote the
  vector defined by $X^{\sqrt{}}_i = X_i^{1/2}.$
  We have
  \begin{eqnarray}
      \max(\sum_i X_i, \sum_i Y_i) & = & \max (\sum_i (X_i^{1/2})^2, \sum_i ({Y_i}^{1/2})^2)  \nonumber \\
                                   & = & \max (||X^{\sqrt{}}||_2^2, ||Y^{\sqrt{}}||_2^2)  \nonumber \\
                                   & \geq & \left((||X^{\sqrt{}}||_2^2, ||Y^{\sqrt{}}||_2^2) \right)^{1/2}  \label{eq:gm1} \\
                                   & = & ||X^{\sqrt{}}||_2 ||Y^{\sqrt{}}||_2  \nonumber \\
                                   & \geq & (X^{\sqrt{}})^T (Y^{\sqrt{}}) \label{eq:cs} \\
                                   & = & \sum_i A_i/\sqrt{C_i(B_i-C_i)} \nonumber \\
                                   & \geq & \frac{2A_i}{B_i} \label{eq:gm2}
  \end{eqnarray}
\end{proof}
\end{comment}


\begin{lemma}
 Let $A,B$ be positive vectors. For all positive vectors $C<B$, and all $0<t<1$, we have
 $$
     \sum_i \frac{A_i}{B_i} \leq \max \left(\sum_i  \frac{tA_i}{C_i}, \sum_i \frac{(1-t)A_i}{B_i-C_i}\right)
 $$
\end{lemma}
\begin{proof}
 Fix an arbitrary $t$. Let
 $$
     f(X) = \max \left(\sum_i  \frac{tA_i}{X_i}, \sum_i \frac{(1-t)A_i}{B_i-X_i}\right)
 $$
We want to study the minimum of $f(X)$ and show it is equal to $\sum_i A_i/B_i$. If we set $X_i=t A_i$ we get that
$$
    \min f(X) \leq  \sum_i \frac{A_i}{B_i}.
$$
We have $X_i<B$ and we can also suppose without loss of generality that $X_i\geq c$
for some sufficiently small $c>0$, because of the lower bound we have on $\min_X f(X)$.
Because the domain is compact, and $f(X)$ is continuous the function attains its minimum.
We claim that the minimum is attained at a point $X$ which satisfies
$$\sum_i  \frac{tA_i}{X_i} = \sum_i \frac{(1-t)A_i}{B_i-X_i}.$$
Suppose for the sake of contradiction that $X$ doesn't satisfy this property.
Then we construct a new vector $X'$ by changing a single coordinate $j$ of $X$ to
$X_j'\Rightarrow X_i-\epsilon$. For sufficiently small $|\epsilon|$ we get $f(X')< f(X)$,
a contradiction.

So, given the constraint, we have
$$
     f(X) = \sum_i \frac{tA_i}{X_i}.
$$
To find the minimum of $f(X)$ under the constraint we will use the method
of Lagrange multipliers. We let $\lambda$ be a new variable and set
$$
    g(X) = - \sum_i \frac{tA_i}{X_i} + \sum_i \frac{(1-t)A_i}{B_i-X_i}.
$$
The minimum must be attained at a point which satisfies for each $i$:
\begin{eqnarray*}
    \frac{\partial f(X)}{\partial X_i} + \lambda \frac{\partial g(X)}{\partial X_i} =0 & \Rightarrow \\
    -\frac{tA_i}{X_i^2} + \lambda\left(\frac{tA_i}{X_i^2} + \frac{(1-t)A_i}{(B_i-X_i)^2} \right) = 0 & \Rightarrow \\
    (\lambda-1)\frac{tA_i}{X_i^2} + \lambda \frac{(1-t)A_i}{(B_i-X_i)^2}=0
\end{eqnarray*}
To solve this system of equations, we can set set $X_i = \phi_i B_i$ and solve for $\phi_i$.
We get
\begin{eqnarray*}
     (\lambda-1)\frac{tA_i}{\phi_i^2 B_i^2} + \lambda \frac{(1-t)A_i}{(1-\phi_i)^2B_i^2} & = & 0  \Rightarrow \\
     (\lambda-1)\frac{t}{\phi_i^2} + \lambda \frac{(1-t)}{(1-\phi_i)^2} & = & 0   \Rightarrow \\
     \lambda\left(\frac{t}{\phi_i^2}+\frac{1-t}{(1-\phi_i)^2}\right) & = & \frac{t}{\phi_i^2}  \Rightarrow  \\
     \frac{\phi_i^2}{(1-\phi_i)^2}  & =  & (\frac{t}{\lambda} -1)/(1-t)
\end{eqnarray*}
From this we get that for all $i,j$
$$
     \frac{\phi_i^2}{(1-\phi_i)^2 } =  \frac{\phi_j^2}{(1-\phi_j)^2} \Rightarrow \frac{\phi_i}{1-\phi_i} = \pm
     \frac{\phi_j}{1-\phi_j},
$$
which implies that $\phi_i=\phi_j=\phi$.
It can be seen that if $\phi>t$
we have for all $i$
$$
    \frac{tA_i}{X_i} < \frac{(1-t)A_i}{B-X_i},
$$
and so $g(x)=0$ doesn't hold. Similarly, we can't have $\phi<t$.  So it must be $\phi=t$.
This also gives us $\lambda = 1-t$ if we solve for $\lambda$. Because there is a unique point $(X,\lambda)$
that satisfies the equations, it must correspond to the minimum. By substituting $X_i=tA_i$ we  get
$$
    \min f(X) = \sum_i \frac{A_i}{B_i}.
$$
\end{proof}

An alternative way of stating the above Lemma is as follows
\begin{lemma} \label{lem:tracediag}
 Let $A,B,C$ be positive vectors. For any $0<t<1$, we have
 $$
    \sum_i \frac{A_i}{B_i+C_i} \leq \max \left( \frac{tA_i}{B_i}, \frac{(1-t)A_i}{C_i} \right)
 $$
\end{lemma}

Now let $A,B$ be positive matrices with the same null space.
We denote by $\lambda_i(A,B)$ the $i^{th}$ largest eigenvalue of
the generalized eigenvalue problem $Ax=\lambda Bx$.
It is well understood that $0$ is a generalized eigenvalue of the pair $(A,B)$
with multiplicity equal to the dimension of the common null space
and all remaining eigenvalues are positive.
We let $trace(A,B)$ denote the trace of the matrix $B^+A$,
where $B^+$ is the Moore-Penrose pseudoinverse of $B$. That is, we have
$$
   trace(A,B) = trace(B^+A) = \sum_i (B^+A)_{ii} =  \sum_i = \lambda_i(A,B),
$$
where the last equality is a well known identity for the trace.

\begin{theorem} \label{th:traceinequality}
 Let $A,B,C$ be positive semi-definite matrices with the same null space. For any $0<t<1$, we have
 $$
    trace(A,B+C) \leq \max \left( trace(tA,B), trace((1-t)A,C) \right).
 $$
\end{theorem}
\begin{proof}
 The matrices  $B$ and $C$ are simultaneously diagonalizable by an invertible matrix $X$
 whose columns are the generalized eigenvectors of the pair $(B,C)$.
 \cite{Stewart.Sun}. That is, there are diagonal matrices $D_A,D_B$ such that
 $$
     X A X^{-1} = D_A \textnormal{~~~and~~~} X B X^{-1} = D_B.
 $$
 Note that we can arrange $X$ so that the first $k$ diagonal entries of $D_A$ and $D_B$
 are 0, and all the remaining ones are positive. Here $k$ is the dimension of the common
 null space.
 We have
 \begin{eqnarray*}
      Az &  =  & \lambda(B+C) z \Rightarrow \\
      X A z & = &  \lambda X(B+C)z \Rightarrow  \\
      X A X^{-1}(Xz) & = & \lambda X(B+C) X^{-1}(Xz) \\
      X A X^{-1}(Xz) &  =  & \lambda (D_B+D_C) (Xz)
 \end{eqnarray*}
Let us set $A_X = XAX^{-1}$. Note that because $A$ has the same
null space with $B,C$, the first $k$ columns and rows of $A_X$ are zero.
The above equality means that  eigenvalues of the pair $(A,B+C)$ are the same as
those of $(A_X,D_B+D_C)$ and thus we have
$$
    trace(A,B+C) = trace(A_X,D_B+D_C)= trace((D_B+D_C)^+ A_X)
$$
Let us denote the lower $(n-k)\times(n-k)$ block of $D_B,D_C, A_X$
respectively by $B',C',A_X'$ respectively. Also let us
denote by $D_A'$ the diagonal of $A_X'$.
Using this notation we have
$$
    trace\left((D_B+D_C)^+ A_X\right) = trace\left( (D_B'+D_C')^{-1} A_X'\right) = trace\left((D_B'+D_C')^{-1} D_A'\right)
$$
where the last equality comes from the fact that $(D_B'+D_C')^{-1}$ is diagonal.
So we have shown that
$$
    trace(A,B+C) = trace\left((D_B'+D_C')^{-1} D_A'\right) = trace(D_A',D_B'+D_C').
$$
Similarly, we can show that
$$
    trace(tA,B) = trace(tD_A',D_B') \textnormal{~~~and~~~} trace((1-t)A,C) = trace((1-t)D_A',D_C').
$$
So to prove the claim it is enough to show that
$$
    trace(D_A',D_B'+D_C') \leq \max \left(trace(tD_A',D_B') ,trace((1-t)D_A',D_C')  \right).
$$
This follows from  Lemma \ref{lem:tracediag} and the fact that $D_A',D_B',D_C'$ are diagonal.
 \end{proof}

We will need the following.

\begin{lemma} \label{th:splittingtrace}
 Let $A$ and $B_i$ be positive semi-definite matrices with the same null space. We have
 $$
      trace(A,\sum_{i=1}^m B_i) \leq \max_i trace(A,mB_i).
 $$
\end{lemma}
\begin{proof}
 We use induction on $m$. The case $m=1$ is trivial.
 By Theorem \ref{th:traceinequality} we have
 \begin{equation} \label{eq:firstsplit}
    trace(A,B_n + \sum_{i=1}^{m-1} B_i) \leq \max \left( trace(A,m B_1), trace( (m-1) A, m \sum_{i=1}^{m-1} B_i) \right)
 \end{equation}
 By the inductive hypothesis we have
 \begin{eqnarray*}
    trace(A,\sum_{i=2}^m B_i) & \leq &  \max_{i>1} trace(A,(m-1)B_i) \Rightarrow \\
    trace((m-1) A,\sum_{i=2}^m B_i) & \leq &  \max_{i>1} trace(A,B_i) \Rightarrow \\
     trace((m-1) A,m \sum_{i=2}^m B_i) & \leq &  \max_{i>1} trace(A,m B_i).
 \end{eqnarray*}
 By plugging this into inequality \ref{eq:firstsplit} we get the inequality.
\end{proof}



